The Best of Both Worlds: Combining Human and Machine Translations for Multilingual Semantic Parsing with Active Learning

Multilingual semantic parsing aims to leverage the knowledge from the high-resource languages to improve low-resource semantic parsing, yet commonly suffers from the data imbalance problem. Prior works propose to utilize the translations by either humans or machines to alleviate such issues. However, human translations are expensive, while machine translations are cheap but prone to error and bias. In this work, we propose an active learning approach that exploits the strengths of both human and machine translations by iteratively adding small batches of human translations into the machine-translated training set. Besides, we propose novel aggregated acquisition criteria that help our active learning method select utterances to be manually translated. Our experiments demonstrate that an ideal utterance selection can significantly reduce the error and bias in the translated data, resulting in higher parser accuracies than the parsers merely trained on the machine-translated data.

==> app-proof-lemma.tex <==
\subsection{Proof of Lemma 1}
Assume $ P^{q}_e(\vx_t|\vx_s) = \lambda_{q}(\vx_s) P_{\theta}(\vx_{t}|\vx_s) + (1-\lambda_{q}(\vx_s))P_{mt}(\vx_{t}|\vx_s)$, where $0 \leq \lambda_{q}(\vx_s) \leq 1$, if $\lambda_{q+1}(\vx_s) \geq \lambda_{q}(\vx_s)$, then $\KL(P_{e}||P^{q}_{\theta}) \leq \KL(P^{q}_{e}||P_{\theta})$.



\subsection{Proof of Lemma 2}
$\mathbb{E}_{P_e(\vx_{t}|\vx_t)}[\log P_{\theta}(\vy| \vx_s)]$ increases or equal, if $\lambda_{q+1}(\vx_s) \leq \lambda_{q}(\vx_s)$. Assume when $\KL(P_e||P_{\theta}) = 0$, $\mathbb{E}_{P_e(\vx_{t}|\vx_t)}[\log P_{\theta}(\vy| \vx_s)]$ reaches maximum. From Lemma 1, if $\lambda_{q+1}(\vx_s) \geq \lambda_{q}(\vx_s)$, then $\KL(P_{e}||P^{q}_{\theta}) \leq \KL(P^{q}_{e}||P_{\theta})$.
Therefore, $\mathbb{E}_{P^{q+1}_e(\vx_{t}|\vx_t)}[\log P_{\theta}(\vy| \vx_s)] \geq \mathbb{E}_{P^{q}_e(\vx_{t}|\vx_t)}[\log P_{\theta}(\vy| \vx_s)]$.


==> app-proof_back.tex <==
\subsection{Bayesian View of Active Human Translation}

The maximum likelihood estimation objective of our parser is:

\begin{align}
\begin{split}
    & \argmin_{\theta}(\iiint_{\vx_s \in \mathcal{X}_{s}, \vx_t \in \mathcal{X}_{t}, \vy \in \mathcal{Y}} R(\pi_{\theta}(\vx), \vy)P(\vy, \vx_t, \vx_s)\,d\vx_s \,d\vx_t \,d\vy)
  %& =\argmax_{\theta}(\iint_{\vx_s \in \mathcal{X}_{s}, \vx_t \in \mathcal{X}_{t}} \log (P_{\theta}(\vy, \vx_t|\vx_s))P(\vx_s)\,d\vx_s \,d\vx_t) \\
   % & =\argmax_{\theta}(\iint_{\vx_s \in \mathcal{X}_{s}, \vx_t \in \mathcal{X}_{t}} \log (P_{\theta}(\vy|\vx_t)P(\vx_t|\vx_s))P(\vx_s)\,d\vx_s \,d\vx_t)
\end{split}
\end{align}
Therefore, to find the source utterance which contribute most to the training error, the objective to select the utterance is:

\begin{align}
\begin{split}
    & \argmax_{\vx_s}(\iint_{\vx_t \in \mathcal{X}_{t}, \vy \in \mathcal{Y}} R(\pi_{\theta}(\vx), \vy)P(\vy, \vx_t, \vx_s) \,d\vx_t \,d\vy) \\
    & \equiv \argmax_{\vx_s}(\log(\iint_{\vx_t \in \mathcal{X}_{t}, \vy \in \mathcal{Y}} R(\pi_{\theta}(\vx), \vy)P(\vy, \vx_t, \vx_s) \,d\vx_t \,d\vy)) \\
    & = \argmax_{\vx_s}(\log(\iint_{\vx_t \in \mathcal{X}_{t}, \vy \in \mathcal{Y}} R(\pi_{\theta}(\vx), \vy)P(\vy, \vx_t | \vx_s) \,d\vx_t \,d\vy))  + \log P(\vx_s)) \\
    & = \argmax_{\vx_s}(\log(\int_{\vx_t \in \mathcal{X}_{t}} R(\pi_{\theta}(\vx), \vy_{\vx_s})P(\vx_t | \vx_s) \,d\vx_t))  + \log P(\vx_s))
\end{split}
\end{align}


%where $P(\vx_t,\vx_s,\vy)$ is the true joint probability.

%\begin{align}
%    & \log (\int_{\vx_t \in \mathcal{X}_{t}} -P_{\theta}(\vx_t,\vx_s,\vy)\,d\vx_t)\\
%    &  =  \log(\int_{\vx_t \in \mathcal{X}_{t}} -P_{\theta}(\vy|\vx_t) P(\vx_t|\vx_s)\,d\vx_t)  + \log P(\vx_s)
    %&  \geq  \log(\int_{\vx_t \in \mathcal{X}_{t}} -P_{\theta}(\vy|\vx_t) P(\vx_t|\vx_s)\,d\vx_t)  + \log P(\vx_s)
    %&  \geq  -\log(\int_{\vx_t \in \mathcal{X}_{t}} P_{\theta}(\vy|\vx_t) P^{q+1}_{e}(\vx_t|\vx_s)\,d\vx_t)  + \log P(\vx_s)
%\end{align}

Let $P^{q+1}_{e}(\vx_t|\vx_s) = \lambda_{q+1} P_{ht}(\vx_{t}|\vx_s) + (1-\lambda_{q+1})P_{mt}(\vx_{t}|\vx_s)$ be the conditional probability at $(q + 1)$th round after the annotation of $\vx_s$, $P^{q}_{e}(\vx_t|\vx_s)=\lambda_{q} P_{ht}(\vx_{t}|\vx_s) + (1-\lambda_{q})P_{mt}(\vx_{t}|\vx_s)$ be the conditional probability at $q$th round, where $\lambda$ is the coefficient between 0 and 1, $1 \geq \lambda \geq 0$ and $\lambda_{q+1} > \lambda_{q}$.

%The inequality between Eq. 9 and Eq. 10 holds because the risk minimization of the parser over the distribution $p_{E}(\mathcal{X}_t|\vx_s,\vy)$. So we make a basic assumption, 
%\begin{align}
%    & \mathbb{E}_{q(\mathcal{X}_t)}(R(\pi_{\theta}(\vx_{t}), \vy)) - \mathbb{E}_{p_{E}(\mathcal{X}_t|\vx_s,\vy)}(R(\pi_{\theta}(\vx_{t}), \vy)) \propto D_{KL}(q(\mathcal{X}_t)||p_{E}(\mathcal{X}_t|\vx_s,\vy))
%\end{align}
%Now the objective turns to maximize $\log(\int_{\vx_t \in \mathcal{X}_{t}} R(\pi_{\theta}(\vx_{t}), \vy)p_{A}(\vx_t|\vx_s,\vy)\,d\vx_t)  + \log p(\vx_s,\vy)$ w.r.t. $(\vx_s,\vy)$.

The lower bound of $\log(\int_{\vx_t \in \mathcal{X}_{t}} R(\pi_{\theta}(\vx), \vy_{\vx_s})P(\vx_t | \vx_s) \,d\vx_t))  + \log P(\vx_s)$ is:

\begin{align}
\begin{split}
    & \log(\int_{\vx_t \in \mathcal{X}_{t}} R(\pi_{\theta}(\vx), \vy_{\vx_s})P^{q+1}_{e}(\vx_t | \vx_s) \,d\vx_t))  + \log P(\vx_s) \\
    &  =  \log(\int_{\vx_t \in \mathcal{X}_{t}}  R(\pi_{\theta}(\vx), \vy_{\vx_s}) \frac{P^{q+1}_{e}(\vx_t|\vx_s)}{Q(\vx_t)} Q(\vx_t))\,d\vx_t)  + \log P(\vx_s) \\
    &  \geq   \mathbb{E}_{Q(\mathcal{X}_{t})}[ \log(R(\pi_{\theta}(\vx), \vy_{\vx_s}) \frac{P^{q+1}_{e}(\vx_t|\vx_s)}{Q(\vx_t)})] + \log P(\vx_s) \\
    &  =   \mathbb{E}_{Q(\mathcal{X}_{t})}[ \log( R(\pi_{\theta}(\vx_{t}), \vy_{\vx_s}))] - \KL({Q(\mathcal{X}_{t})}||P^{q+1}_{e}(\mathcal{X}_t|\vx_s)) + \log P(\vx_s)
    %\text{Likewise:}\\
    %& \log(\int_{\vx_t \in \mathcal{X}_{t}} R(\pi_{\theta}(\vx_{t}), \vy)p_{E}(\vx_t|\vx_s,\vy)\,d\vx_t)  + \log p(\vx_s,\vy)
    %&  \geq   \mathbb{E}_{Q_{E}(\mathcal{X}_{t})}[ \log( R(\pi_{\theta}(\vx_{t}), \vy))] - \KL({Q_{E}(\mathcal{X}_{t})}||p_{E}(\mathcal{X}_t|\vx_s,\vy)) + \log p(\vx_s,\vy)
\end{split}
\end{align}
Let $Q_{E}(\mathcal{X}_{t}) = p_{E}(\mathcal{X}_t|\vx_s,\vy)$ and $Q_{A}(\mathcal{X}_{t}) = p_{A}(\mathcal{X}_t|\vx_s,\vy)$, the two evidence lower bounds (ELBO) are $ELBO_{1} = \mathbb{E}_{p_{E}}[ \log( R(\pi_{\theta}(\vx_{t}), \vy))] + \log p(\vx_s,\vy)$ and $ELBO_{2} = \mathbb{E}_{p_{A}}[ \log( R(\pi_{\theta}(\vx_{t}), \vy))] + \log p(\vx_s,\vy)$. At beginning, since we don't have $p_{A}(\mathcal{X}_t|\vx_s,\vy)$, we aim to maximize the $ELBO_{1}$ first w.r.t $(\vx_s, \vy)$ and we hope, after annotation, the $ELBO_{2}$ can be maximized with the same selected $(\vx_s, \vy)$.
\begin{align}
\begin{split}
    & ELBO_{2} - ELBO_{1} \\
    &  =  \mathbb{E}_{p_{A}}[ \log( R(\pi_{\theta}(\vx_{t}), \vy))]-\mathbb{E}_{p_{E}}[ \log( R(\pi_{\theta}(\vx_{t}), \vy))] 
\end{split}
\end{align}

==> previous_method.tex <==


%In order to mitigate the two issues aforementioned, a small set of human translations can be included in the training set

To mitigate the negative effect of translation bias and error in the MT data, we propose \hatt, which introduces extra human supervision to machine supervision when training the MSPs. Two major intuitions motivate our training approach: 
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
\item Adding the HTs to the training data could enrich its lexical and morphological diversity and ensure that the lexical distribution of the training data is closer to the human test set, thus improving the parsers' generalization ability~\cite{shiri2022paraphrasing,xu2020autoqa,wang2015building}. 
\item Human translations are less erroneous than the machine translations~\cite{freitag2021experts}. The parser could learn to predict  correct abstractions with  less erroneous training data.
\end{itemize}
%In our active learning setting, we assume access to a well-trained machine translation system and a semantic parsing dataset with utterances in a source language $l_s$ (e.g. English) paired with logical forms, $\mathcal{D}_s = \{(\vx^{s}_i, \vy_i)\}_{i=1}^{N}$. Each utterance $\vx^{s}$ in $\mathcal{D}_s$ is translated into the utterance $\vx^{m}$ in the target language $l_t$ by the MT system, $\mathcal{D}_{t,m} = \{(\vx_i^{t,m}, \vy_i)\}_{i=1}^{N}$. With a semantic parser initially trained on the the combination of two datasets $\mathcal{D}_s \cup \mathcal{D}_{t,m}$, the goal of our active learning method is to sample a small set of $K_q$ examples in the $q$th sampling round from the training set in the source language, $\mathcal{D}'_s \in \mathcal{D}_s$ and translate them into target language with human translators, $\mathcal{D}^{q}_{t,h} = \{(\vx^{t,h}_i, \vy_i)\}_{i=1}^{K_q}$. The selection criterion is based on the \textit{acquisition functions}, which are used to score the examples in the source language. Following the conventional active learning setting~\cite{}, there are $Q$ rounds of selection, thus the size of $\mathcal{D}_{t,h} = \bigcup^{Q}_{q=1} \mathcal{D}^{q}_{t,h}$ is incrementally increasing.  The detailed active learning procedure iteratively performs the following steps:

Our \hatt active learning setting considers only the \textit{bilingual} scenario, one of which is the high-resource language and the other one is in low-resource. However, it is easy to extend our method to more than two languages. We assume access to a well-trained black-box multilingual MT system, $g^{mt}(\cdot)$, and a semantic parsing training set that includes utterances in a high-resource language $l_s$ (e.g. English) paired with LFs, $\mathcal{D}_s = \{(\vx_{s}^i, \vy^i)\}_{i=1}^{N}$, two human-generated test sets $\mathcal{T}_{s} = \{(\vx_{s}^i, \vy^i)\}_{i=1}^{M}$ and $\mathcal{T}_{t} = \{(\vx_{t}^i, \vy^i)\}_{i=1}^{M}$ with utterances in high and low-resource languages, respectively. Each utterance $\vx_{s}$ in $\mathcal{D}_s$ is translated into the utterance $\hat{\vx}_{t} = g^{mt}_{s\rightarrow t}(\vx_{s})$ in the target language $l_t$ by the MT system, $\hat{\mathcal{D}}_{t} = \{(\hat{\vx}^i_{t}, \vy^i)\}_{i=1}^{N}$. With a semantic parser initially trained on the combination of source data and the MT data, $\mathcal{D}^{0} = \mathcal{D}_s \cup \hat{\mathcal{D}}_{t}$, the goal of our active learning method is to select a small set of utterances from the training data in the source language, $\tilde{\mathcal{D}}_s \in \mathcal{D}_s$, and translate the utterances in $\tilde{\mathcal{D}}_s$ to the target language by the human translators, $\bar{\mathcal{D}}_t = g^{ht}_{s\rightarrow t}(\tilde{\mathcal{D}}_s)$. 


The selection criterion is based on the \textit{acquisition functions} that score the source utterances. Following the conventional batch AL setting~\cite{duong2018active}, there are $Q$ rounds of selection. At $q$th round, AL selects utterances with a budget size of $K_q$.
%thus the size of $\mathcal{D}_{t,h} = \bigcup^{Q}_{q=1} \mathcal{D}^{q}_{t,h}$ is incrementally increasing. 
The detailed \hatt active learning procedure iteratively performs the following steps as in Algorithm.~\ref{algo:al}.% at the $q$th query round:

%\noindent\textbf{Step1}: Train the semantic parser $P_{\theta}(\vy|\vx)$ to convergence over the training data, $\mathcal{D}^{q} = \mathcal{D}_s \cup \hat{\mathcal{D}}_t \cup \mathcal{D}^{1:q-1}_t$, which is the combination of data in the source language $\mathcal{D}_s$, machine-translated data $\hat{\mathcal{D}}_t$ and the human-translated data from previous query rounds $\mathcal{D}^{1:q-1}_t = \bigcup^{q-1}_{i=1} \mathcal{D}^{i}_{t}$ if there are any.

%\noindent\textbf{Step2}: With our active learning acquisition functions, select a subset $\tilde{\mathcal{D}}^{q}_s$ in size of $K_q$ from the source language data. The human annotators translate the utterances in $\tilde{\mathcal{D}}^{q}_s$ into the target language, $\mathcal{D}^{q}_t = g^{ht}_{s\rightarrow t}(\tilde{\mathcal{D}}^{q}_s)$.

%\noindent\textbf{Step3}: Add the human-translated data into the training data, $\mathcal{D}^{1:q}_t = D^{1:q-1}_t \bigcup D^{q}_{t}$ and repeat Step1-Step3 until the $Q$ rounds of sample selection are performed.

\input{algo-al}


%An LF $\vy = \{\vy_{s}^1,...,\vy_{s}^n\}$ can be further decomposed into a set of sub-structures, each of which $\vy_{s}^n = (\vv_{s}^{n}, \ve_{s}^{n})$ is constructed by the subset of the node set $\vv_{s}^{n} \subseteq \vv$ and the edges linking the nodes $\ve_{s}^{n} \subseteq \vv_{s}^{n} \times \vv_{s}^{n} $.

%Each task $\mathcal{T}^{(k)}$ includes its own training/validation/test set ($\mathcal{D}^{(k)}_{train}$,$\mathcal{D}^{(k)}_{valid}$,$\mathcal{D}^{(k)}_{test}$), each of which is a set of utterance-LF pairs $(\mathcal{X}^{(k)}, \mathcal{Y}^{(k)})$. The \textit{boundaries} between tasks are defined by \textit{task descriptors}~\cite{lopez2017gradient}, which provides contextual information about examples $(\mathcal{X}^{(k)}, \mathcal{Y}^{(k)})$ in each task. For example, the descriptors might describe that each task belongs to a distinct domain, or the questions $\mathcal{X}^{(k)}$ in each task are in a unique set of types or querying about a distinct set of cities. The node set $\mathcal{V}^{(k)} = \mathcal{V}^{(k)}_{s} \cup \mathcal{V}_g $ in the LFs $\mathcal{Y}^{(k)}$ of each task $\mathcal{T}^{(k)}$ can be further divided into task-specific nodes $\mathcal{V}^{(k)}_{s}$ and task-general nodes $\mathcal{V}_{g}$. The task-specific nodes $\mathcal{V}^{(k)}_{s}$ only exist in $k$-th task while the task-general nodes $\mathcal{V}_{g}$ are shared across different tasks \reza{among tasks seen so far?}. 
%As an example in Table , the nodes, "" and "", in LFs from two different tasks, "" and "", are distinct in each task, while the rest nodes are shared by two LFs. 
%Task-specific nodes $\mathcal{V}_{s}$ usually possess semantics related to descriptors, such as entities in each domain, question types or city names.
% to do a table showing two LFs from different tasks.
\subsection{Acquisition Functions} 
\label{sec:acq}
%\textbf{Hypothesis:} \textit{The diversified and representative source utterances in the training set that also have biased and erroneous translations could mitigate the translation bias and error problems in the overall dataset to the greatest extent.}
%The acquisition functions are designed based on our intuitions to mitigate the translation errors and translation bias. Formally, the active learning problem is to sample and annotate a small set of examples to minimize the future risk~\cite{}. Since this target is difficult to achieve, many current works reformulate this problem into sampling the examples that could maximize the total risk of the models after annotation. In our problem, the objective when we select each example turns to:

% \begin{small}
% \begin{align}
%     \argmax_{\vx_s,\vy}\iint R(\pi_{\theta}(\vx_{t}), \vy)p(\vx_t,\vx_s,\vy)\,d\vx_t \,d\vy
% \end{align}
% \end{small}

%\noindent\ignorespaces where $p_{D}(\vx_t,\vx_s,\vy)$ is the distribution of the the training data $D$, which includes source language data, MT translated data and human translated data. With a simple Bayesian factorization,

% \begin{small}
% \begin{align}
%     p(\vx_t,\vx_s,\vy) = \frac{p(\vx_t,\vx_s,\vy)}{p_{D}(\vx_t,\vx_s,\vy)}p_{D}(\vx_t,\vx_s,\vy)
% \end{align}
% \end{small}

% \noindent\ignorespaces If we assume the $p_{D}(\vx_s,\vy)$ is the same as the true distribution of the source language data since $\vs_s$ is the human data, we can see the objective becomes:
% \begin{small}
% \begin{align}
% \label{eq:obj}
%     \argmax_{\vx_s,\vy}\iint R(\pi_{\theta}(\vx_{t}),\vy) \frac{p(\vx_t|\vx_s,\vy)}{p_{D}(\vx_t|\vx_s,\vy)}p_{D}(\vx_t,\vx_s,\vy)\,d\vx_t \,d\vy
% \end{align}
% \end{small}

%Given our hypothesis to mitigate translation bias and errors, we derive four acquisition functions for selecting the utterances. Then, we aggregate the four acquisition functions to acquire their joint benefits. 
%The acquisition functions score the utterances. 
The acquisition functions assign higher scores to those utterances whose HTs  can boost the parser's performance more than the HTs of the other utterances.
%human translations of the selected utterances with the higher scores should boost the multilingual parsers' performance more than the others. 
The prior AL works~\cite{sener2018active,zhdanov2019diverse,nguyen2004active} suggest that the most representative and diversified examples in the training set improve the generalization ability of the machine learning models the most. Therefore, we provide a hypothesis that \textit{we should select the representative and diversified utterances in the training set, whose  current translations have significant bias and errors}. We postulate fixing problems of such utterances improves the parsers' performance the most. We derive four acquisition functions based on this hypothesis to score the utterances. Then, \amsp aggregates these acquisition functions to gain their joint benefits. In each AL round, the utterances with the highest \amsp scores are selected.

\noindent\textbf{Translation Bias.} 
%The term $\frac{p(\vx_t|\vx_s,\vy)}{p_{D}(\vx_t|\vx_s,\vy)}$ in Eq. \ref{eq:obj} implys that the $\vx_s$ with the largest translation bias should be selected. However, true distribution $p(\vx_t|\vx_s,\vy)$ is usually unknown. Therefore, here we made an assumption $p(\vx_t|\vx_s,\vy)$ is in an uniform distribution since the human translations are more diversified.
We assume an empirical conditional distribution, $P_{e}^{q}(\vx_t|\vx_s)$, for each utterance $\vx_s$ in $\mathcal{D}_{s}$ at $q$th AL selection round. The empirical conditional distribution is considered as a mixture of distributions from  the human  $P_{ht}(\vx_{t}|\vx_s)$ and machine $P_{mt}(\vx_{t}|\vx_s)$. \reza{Why the empirical distribution is defined in this particular way as a mixture of these two distributions? Is it 'assumed' or is it 'proved'? If assumed, what is the basis for this assumption?} %$P_{e}^{q}(X_{t}|\vx_s) = \lambda^{\vx_s}_{q} P_{ht}(X_{t}|\vx_s) + (1-\lambda^{\vx_s}_{q})P_{mt}(X_{t}|\vx_s)$, where $\lambda_{q}^{\vx_s}$ is a coefficient between 0 and 1. 
%After annotation of $x_s$ at each round, $P_{e}^{q}(\mathcal{X}_{t}|\vx_s)$ is more close to the human translation distribution

%over the source and target utterances in the training data, $\mathcal{D}^{q}$ at $q$th round.
Intuitively, the $\vx_s$ with the most biased translations should be the one with the most skewed empirical conditional distribution. Therefore, we measure the translation bias by calculating the entropy of the empirical conditional distribution, $H(P_{e}^{q}(\vx_{t}|\vx_s))$, and select the $\vx_s$ with the lowest entropy. Since the translation space  $\mathcal{X}_{t}$ is exponentially large, it is intractable to directly calculate the entropy. Following ~\cite{settles-craven-2008-analysis}, we adopt two approximation strategies, \textit{N-best Sequence Entropy} and \textit{Maximum Confidence Score}, to approximate the entropy.

%over the current training set $\mathcal{D}$.
\noindent\textit{$\bullet$ N-best Sequence Entropy:}

\begin{small}
\begin{align}
    \phi_b(\vx_s) = - \sum_{\hat{\vx}_t \in \mathcal{N}} \hat{P_{e}^{q}}(\hat{\vx}_t|\vx_s) \log \hat{P_{e}^{q}}(\hat{\vx}_t|\vx_s)
\end{align}
\end{small}

\noindent\ignorespaces where $\mathcal{N} = \{\hat{\vx}^{1}_t,...,\hat{\vx}^{N}_t\}$ are the $N$-best hypothesis sampled from the empirical distribution $P_{e}^{q}(\vx_{t}|\vx_s)$. $\hat{P_{e}^{q}}(\hat{\vx}_t|\vx_s)$ is re-normalized from $P_{e}^{q}(\hat{\vx}_t|\vx_s)$ over $\mathcal{N}$, which is only a subset of $\mathcal{X}_{t}$.

%Though we could use a seq2seq model to estimate each $p_{D}(\vx_t|\vx_s,\vy)$, we adopt the IBM1 model~\cite{} to reduce the model training time. Heuristically, the more probable translations the $\vx_s$ has, the less likely it will be selected given this term. More probable translations also imply that $\vx_s$ have more diversified translations than the others.

%A direct way to estimate the empricial distribution $p(\vx_t|\vx_s)$ is to use a machine translation model. However,  Instead, we estimate $\sum_{\vy \in \mathcal{Y}} p(\vx_t|\vy) p(\vy|\vx_{s})$. Since $p(\vy|\vx_{s})$ is deterministic, we use a Seq2Seq model to estimate $p(\vx_t|\vy)$.


\noindent\textit{$\bullet$ Maximum Confidence Score (MCS)}:

% \begin{small}
% \begin{align}
%     \phi_b(\vx_s) & = -\frac{1}{|\vy|} \sum_{y_i \in \vy} H(p(\mathcal{V}_{t}|y_{i})) \\
%     s.t. \vy & = \argmax_{\vy} p(\mathcal{Y}|\vx_s)
% \end{align}
% \end{small}


\begin{small}
\begin{align}
    \phi_b(\vx_s) & =  \log P_{e}^{q}(\vx'_t|\vx_s) \\
    s.t. \vx'_t & = \argmax_{\vx_t} P_{e}^{q}(\vx_{t}|\vx_s)
\end{align}
\end{small}
\noindent\ignorespaces It is difficult to obtain the empirical distribution as we know neither of the two distributions that compose the empirical distribution. Therefore, we use distillation training~\cite{hinton2015distilling} to train a translation model that estimates $P_{e}^{q}(\vx_t|\vx_s)$ on all the bilingual pairs $(\vx_s, \vx_t)$ in the MSP training data $\mathcal{D}^{q}$. Another challenge is that $\mathcal{D}^{q}$ is too small to distil a good translation model that imitates the mixture distribution. Here, we apply a bayesian factorization trick that factorizes $P_{e}^{q}(\vx_{t}|\vx_s) = \sum_{\vy \in \mathcal{Y}} P_{e}^{q}(\vx_t|\vy) P_{e}^{q}(\vy|\vx_{s})$, where $y$ ranges over LFs representing the semanics. As there is a deterministic mapping between $\vx_s$ and the LF, $P_{e}^{q}(\vy|\vx_{s})$ is an one-hot distribution. Thus, We only need to estimate the entropy, $H(P^{q}_{e}(\vx_t|\vy))$. This has  a nice intuition:  the less diversified data has less lexically diversified utterances per each LF. Note that if we use this factorization, all $\vx_s$ that share the same LF have the same scores. 

%As in Fig.~\ref{fig:factorization_al_result} at Appendix~\ref{app:abl_fact}, at several query rounds, the parser accuracy can be 3\% - 6\% higher than that using no factorization in \textit{N-best Sequence Entropy}.

We use the lightweight Seq2Seq model to estimate $P_{e}^{q}(X_t|\vx_s)$ or $P^{q}_{e}(\vx_t|\vy)$. 
%, which only takes around 30s on \geo to train the model. 
Ideally, every time a new source utterance $\vx_s$ is selected, $P_{e}^{q}(\vx_t|\vx_s)$ should be re-estimated. However, we only re-estimate $P_{e}^{q}(\vx_t|\vx_s)$ once at the beginning of each selection round to reduce the training cost.

%It is difficult to obtain the empirical distribution as we know neither of the two distributions that compose the empirical distribution. We adopt 

%A direct way to estimate the empirical distribution $P_{e}^{q}(X_t|\vx_s)$ is to train a machine translation model (i.e. a statistical model or a neural Seq2Seq model) on the translation pairs $(\vx_s, \vx_t)$ in $\mathcal{D}^{q}$. However, since empirical distribution is the mixture of two complicated distributions, the distribution of human translation and the distribution of the machine translation service., $\mathcal{D}^{q}$ is too small to train a decent translation model that estimates the empirical distribution. Instead, we use a bayesian factorization trick that factorizes $P_{e}^{q}(\vx_{t}|\vx_s) = \sum_{\vy \in \mathcal{Y}} P_{e}^{q}(\vx_t|\vy) P_{e}^{q}(\vy|\vx_{s})$. Since $P_{e}^{q}(\vy|\vx_{s})$ is one-hot, we only need to estimate $P^{q}_{e}(\vx_t|\vy)$. The intuition behind is straightforward. The more diversified data should have more lexically diversified utterances per each LF. Note that if we use this factorization, all $x_s$ that share the same LF will have same scores. Empirically, we found the bias acquisition functions using the factorization performs much better. 

%We use the lightweight Seq2Seq model to estimate $P_{e}^{q}(X_t|\vx_s)$, which only takes around 30s on \geo to train the model. Ideally, every time a new source utterance $\vx_s$ is selected, $P_{e}^{q}(X_t|\vx_s)$ should be re-estimated. However, we only re-estimate $P_{e}^{q}(X_t|\vx_s)$ once at the beginning of each selection round to reduce the training cost.
%where $\mathcal{V}_{t}$ is the vocabulary extracted from training set $\mathcal{D}$ in the target language
\noindent\textbf{Translation Error.} 
Similar to~\cite{haffari-etal-2009-active}, we leverage back-translations to measure the translation error. We conjecture that if the translation quality for one source utterance $\vx_s$ is good enough, the semantic parser should be confident in the LF of the source utterance conditioned on its back-translations. %In other words, if the parser is not confident in its parsing result, $\vx_s$ most likely has translation errors. 
Therefore, we measure the translation error for each $\vx_s$ as the expected parser's negative log-likelihood in its corresponding LF $\vy_{\vx_s}$ over all the back-translations of $\vx_s$, $\mathbb{E}_{P^{q}_{e}(X_{t}|\vx_s)}[-\log(P^{q}_{\theta}(\vy_{\vx_s}|g_{t \rightarrow s}^{mt}(\vx_t)))]$, where $P^{q}_{\theta}$ is the parser trained at $q$th round. To approximate the expectation, we apply two similar strategies as mentioned in \textit{Translation Bias}.
%$\vy_{\vx_s}$ is the corresponding LF of $\vx_s$, $g_{t \rightarrow s}^{mt}$ is the back-translation model and
%The maximize the risk of the parser over the $\vx_t$, $R(\pi_{\theta}(\vx_{t}),\vy)$, one direct way is to select the examples in the source language with translation errors. Since it is difficult to measure the translation error between $\vx_s$ and its corresponding MT translation $\vx_{t,m}$. We provide an indirect way to measure the translation error using the trained semantic parser:

\noindent\textit{$\bullet$ N-best Sequence Expected Error:}

\begin{small}
\begin{align}
    \phi_e(\vx_s) & = -\sum_{\hat{\vx}_t \in \mathcal{N}_{\vy_{\vx_s}}} \hat{P}_{e}^{q}(\hat{\vx}_t|\vx_s) \log P_{\theta}(\vy_{\vx_s}|g_{t \rightarrow s}^{mt}(\vx_t)) 
\end{align}
\end{small}

\noindent\ignorespaces where $\mathcal{N}_{\vy_{\vx_s}}$ is the set of translations in $\mathcal{D}^q$ that share the same LF $\vy_{\vx_s}$ with $\vx_s$. We only back-translate utterances in $\mathcal{D}^q$ to reduce the cost of back-translations.

%where $\vx'_s = g^{-1}_{mt}(\vx_t)$ is the back-translation of $\vx_s$ with $\vx_{t} = g_{mt}(\vx_s)$ as its bridge utterance, $\mathcal{M}_{\vy}$ includes $\vx_t$ that shares the same $\vy$ with $\vx_s$. A direct way to estimate the empirical distribution $p(\vx_t|\vx_s)$ is to use a machine translation model. However,  Instead, we factorize $\sum_{\vy \in \mathcal{Y}} p(\vx_t|\vy) p(\vy|\vx_{s})$. We use a Seq2Seq model to estimate $p(\vx_t|\vy)$. We assume that if the translation is not correct, the parser will not be able to parse its corresponding back-translation correctly.

\noindent\textit{$\bullet$  Maximum Error:}

\begin{small}
\begin{align}
    \phi_e(\vx_s) & = - \log P^{q}_{\theta}(\vy_{\vx_s}|g^{mt}_{t \rightarrow s}(\vx'_t)) \\
        s.t. \vx'_t & = \argmax_{\vx_t} P^{q}_{e}(\vx_{t}|\vx_s)
\end{align}
\end{small}

\noindent\ignorespaces We use the same distilled translation model $P^{q}_{e}(\vx_{t}|\vx_s)$ used in \textit{Translation Bias}.

%where $\vx_t$ is obtained by $\vx_t = \argmax_{\vx_t} p_{E}(\mathcal{X}_{t}|\vx_s)$. We don't need to train any model here since $\argmax_{\vx_t} p_{E}(\mathcal{X}_{t}|\vx_s)$ is already provided by MT model, $\vx_t = g_{mt}(\vx_s)$. After annotation, the $\argmax_{\vx_t} p_{E}(\mathcal{X}_{t}|\vx_s)$ is presumed to be the human translation.
%Shannon's diversity index

\noindent\textbf{Semantic Density.}
The previous AL works~\cite{nguyen2004active,donmez2007dual} have found that the most \textit{representative} examples improve the model performance the most. Therefore we desire to reduce the translation error and bias for the translations of the most representative source utterances. As such,  the utterances should be selected from the dense regions in the semantic space,
\begin{equation}
    \phi_s(\vx_s) = \log P(\vx_s).
\end{equation}
We use kernel density estimation~\cite{botev2010kernel} with the exponential kernel to estimate $P(\vx_s)$, while other density estimation methods could be also used. The feature representation of $\vx_s$ for density estimation is the average pooling of the contextual sequence representations from the MSP encoder. The density model is re-estimated at the beginning of each query selection round.

\noindent\textbf{Semantic Diversity.} The role of the semantic diversity function is twofold. First, it prevents the AL method from selecting similar utterances. Resolving the bias and errors of similar utterances in a small semantic region does not resolve the training issues for the overall dataset. Second, semantic diversity correlates with the lexical diversity, hence improving it also enriches lexical diversity.
\begin{align}
    \phi_d(\vx_s) =     
    \begin{cases}
      0 & \text{if $c(\vx_s) \notin \bigcup_{\vx^{i}_s \in \mathcal{S}} c(\vx^{i}_s)$}\\
      -\infty & \text{Otherwise}
    \end{cases}
\end{align}
\noindent\ignorespaces where $c(\vx_s)$ maps each utterance $\vx_s$ into a cluster id and $\mathcal{S}$ is the set of cluster ids of the selected utterances. We use a clustering algorithm to diversify the selected utterances as in~\cite{ni2020merging,nguyen2004active}. The source utterances are partitioned into $|\mathcal{C}|$ clusters. We select one utterance at most from each cluster. Notice the number of clusters should be greater than or equal to the total budget size until current selection round, $|\mathcal{C}| \geq \sum^{q}_{i=1}K_{i}$. The clusters are re-estimated every round. To ensure the optimal exploration of semantic spaces across different query rounds, we adopt Incremental K-means~\cite{liu2020active} as the clustering algorithm. At each new round, Incremental K-means considers the selected utterances as the fixed cluster centres, and learns the new clusters conditioned on the fixed centres. The feature representation of $\vx_s$ for Incremental K-means is from MSP encoder as well.

\noindent\textbf{Aggregated Acquisition.}
We aggregate the four acquisition functions into one,
\begin{align}\nonumber
\label{eq:sample}
    & \phi_{A}(\vx_s) = \sum_{k}\alpha_{k} \phi_{k}(\vx_s) 
    %s.t. & c(\vx_s,\vy) \notin \cup^{|\mathcal{L}|}_{i=1} c(\vx^{i}_s,\vy)
\end{align}
\noindent where $\alpha_{k}$'s are the coefficients. Each $\phi_{k}(\vx_s)$ is normalized using quantile normalization~\cite{bolstad2003comparison}. Given the approximation strategies we used for \textit{Translation Bias} and \textit{Translation Error}, we provide two types of aggregations, \amspnbest and \amspmax. \amspnbest applies \textit{N-best Sequence Entropy} and \textit{N-best Sequence Expected Error}. \amspmax applies \textit{Maximum Confidence Score} and \textit{Maximum Error}.
%\subsection{Hyperparameter Tuning}https://www.overleaf.com/project/61ba0e495e10d29d365bbb65

==> tab-abl-diversity_error.tex <==
\begin{table}[ht]
    \vspace{-2mm}
\centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c|cccc|cccc|c|}
    \toprule
     Metric &  \bias & \error & \density & \diversity &  - \bias & - \error & - \density & - \diversity & \amspnbest  \\
      \midrule
          Error$\uparrow$ &   &  &  &  &  &  &  & & \\
     \hline
    BLEU$\uparrow$ &  - & - & - & - & 19.67 & - & - & - & 19.51 \\
\hline
    Self-BLEU$\downarrow$ & -  & - & - & - & 78.44 & - & - & - &77.80 \\
  MTLD$\uparrow$ & - &  -  & -  & - & 23.86 & - & - & - & 23.86   \\
        \hline
 Simpson Index$\downarrow$ & - & - & - & - &93.24 & - & - & -  & 93.15 \\
    \bottomrule
  \end{tabular}%
  }
    \caption{The scores of three metrics to measure the bias of the human (HT) and machine (MT) translations in \geo and \nlmap in German (De), Thai (Th) and Greek (El). '-' means Simpson Index does not apply to Thai. \vspace{-2mm}}
  \label{tab:abl_diversity_error}
  \vspace{-2mm}
\end{table}

==> tab-abl-diversity_error_back.tex <==
\begin{table}[ht]
    \vspace{-2mm}
\centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c|cccc|cccc|c|}
    \toprule
     Metric &  \bias & \error & \density & \diversity &  - \bias & - \error & - \density & - \diversity & \amspnbest  \\
      \midrule
          Error$\uparrow$ &   &  &  &  &  &  &  & & \\
     \hline
    BLEU$\uparrow$ &  20.27 & 20.13 & 20.59 & 20.04 & 21.46 & 20.20 & 19.69 & 20.11 & 20.72 \\
\hline
    Self-BLEU$\downarrow$ & 74.59  & 74.12 & 77.88 & 76.02 & 76.16 & 76.19 & 75.79 & 79.42 &76.01 \\
  MTLD$\uparrow$ & 35.43 &  35.28  & 34.41  & 34.89 & 35.07 & 34.25 & 34.98 & 35.74 & 35.23   \\
        \hline
 Simpson Index$\downarrow$ & 92.93 & 92.61 & 92.34 & 93.21 &93.00 & 93.15 & 92.83 & 95.65  & 92.91 \\
    \bottomrule
  \end{tabular}%
  }
    \caption{The scores of three metrics to measure the bias of the human (HT) and machine (MT) translations in \geo and \nlmap in German (De), Thai (Th) and Greek (El). '-' means Simpson Index does not apply to Thai. \vspace{-2mm}}
  \label{tab:abl_diversity_error}
  \vspace{-2mm}
\end{table}

==> tab-bt-discrepancy.tex <==
\begin{table}[t]
    % \vspace{-1mm}
\centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c|c|}
    \toprule
    \multicolumn{2}{|c|}{\geode} \\
        \hline
       Original & how many state border at least one other state \\
      Translation & wie man an mindestens einen anderen Staat grenzt  \\
          Back-Translation & how to border at least one other state \\
              \hline
                   \multicolumn{2}{|c|}{\geoth} \\
                       \hline
            Original & what is the area of c0 \\
      Translation & \\
         Back-Translation & c0 . What is the area? \\        
    \bottomrule
  \end{tabular}%
  }
    \caption{The back-translation examples from \geode, \geoel, \geoth and \nlmapde. \vspace{-3mm}}
  \label{tab:back_examples}
    
\vspace{-3mm}
\end{table}

==> tab-correctness.tex <==
\begin{table}[t]
    % \vspace{-1mm}
\centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c||cccc|}
    \toprule
   
      & \geode  & \geoel & \geoth & \nlmapde   \\
       \midrule \midrule
     Mistranslation Rate of BTs & 11\% & 12\% &  10\% &10\% \\
                
    \bottomrule
  \end{tabular}%
  }
    \caption{The mistranslation rates of the back-translations of the English utterances in \geo and \nlmap with German (De), Thai (Th) and Greek (El) as the bridge languages. \vspace{-3mm}}
  \label{tab:change_rate}
    
\vspace{-3mm}
\end{table}

==> tab-diversity_error_back.tex <==
\begin{table}[ht]
    \vspace{-2mm}
\centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c|ccccccc|cc|}
    \toprule
     Metric & \rand & \cluster & \csse & \rttl & \lcsfw & \lcsbw & \traffic & \amspnbest & \amspmax  \\
      \midrule
          Error$\uparrow$ & 11\%  & 14\% & 11\% & 21\% & \textbf{22\%} & 8\% & 14\% & 17\% & 18\% \\
     \hline
    BLEU$\uparrow$ &  20.07 & 20.38 & 19.56 & 20.05 & 18.79 & 18.71 & 19.22 & 20.72 & \textbf{20.91} \\
\hline
    Self-BLEU$\downarrow$ &  78.39 & 79.30 & 78.16 & 77.99 & \textbf{74.93} & 84.57 & 81.26 & 76.01 & 76.37 \\
  MTLD$\uparrow$ & 34.07 &  33.61  & 34.14  & 34.96 & 34.22 & 33.32 & 33.79 & \textbf{35.23} & -    \\
        \hline
 Simpson Index$\downarrow$ & 93.41 & 93.32 & 93.13 & \textbf{91.82} &92.48 & 94.25 & 93.51&  92.91 & 93.06\\
    \bottomrule
  \end{tabular}%
  }
    \caption{The scores of three metrics to measure the bias of the human (HT) and machine (MT) translations in \geo and \nlmap in German (De), Thai (Th) and Greek (El). '-' means Simpson Index does not apply to Thai. \vspace{-2mm}}
  \label{tab:main_diversity_error}
  \vspace{-2mm}
\end{table}
